Semi-stable models of modular Curves $X_0(p^2)$ and some arithmetic applications

In this paper, we compute the semi-stable models of modular curves $X_0(p^2)$ for odd primes $p > 3$ and compute the Arakelov self-intersection numbers of the relative dualising sheaves for these models. We give two arithmetic applications of our computations. In particular, we give an effective version of the Bogomolov conjecture following the strategy outlined by Zhang and find the stable Faltings heights of the arithmetic surfaces corresponding to these modular curves.

==> dualgraph.tex <==
Let $\Gp$ be the dual graph of the special fiber $\cX_0(p^2)_{(\fancyp)}$. This is a metrized
graph in the sense of Zhang \cite{\zhang}. Let $V(\Gp)$ be the set of vertices, and 
$E(\Gp)$ the set of edges of $\Gp$. We denote by $l(\Gp)$ the sum of lengths of all the edges. For any 
$x \in V(\Gp)$, $g(x)$ is the geometric genus of the corresponding component of $\cX_0(p^2)_{(\fancyp)}$.

\subsection{Case $p=12k+1$}
Recall the  diagram for the special fiber is given by Figure \ref{fig:semistable1}. 
We draw the dual graph of the special fiber here. 
In the dual graph we denote the vertices corresponding to the components by small letters with the same indices 
but drop the tildes. We ignore the vertices with genus 0 and valence 2. 
\begin{center}
\includegraphics[scale=0.6]{dual1mod12.pdf}
\end{center}
Each black edge has length $6k$ and green edge has length $1$. None of the edges intersect.
As a consequence, we conclude that $l(\Gp)=12k^2+2k$. 
We have $g(\ell_i) = 6k, \quad g(c_{2,0}) = g(c_{0,2}) = 0, \quad g(c_{1,1}^i) = 3k^2 -3k + 1 $.

\subsection{Case $p=12k+5$}
In this case,  diagram for the special fiber is given by Figure \ref{fig:semistable5}. 
Further $g(c_{2,0}) = g(c_{0,2}) = 0, \quad g(c_{1,1}^i) = 3k^2 - k, \quad g(\ell_i) = 6k+2, 
\quad g(f)= 2k$. The dual graph is the following.
\begin{center}
\includegraphics[scale=0.6]{dual5mod12.pdf}
\end{center}
Black edges have length $6k+2$, orange edges length $18k+6$, blue edges length $3$ and green
are of length $1$. As a consequence, we conclude that $l(\Gp)=12k^2+42k+18$. 

\subsection{Case $p=12k+7$}
In this case,  diagram for the special fiber is given by Figure \ref{fig:semistable7}. 
Further $g(c_{2,0}) = g(c_{0,2}) = 0, \quad g(c_{1,1}^i) = 3k^2, \quad g(\ell_i) = 6k+3, 
\quad g(e)= 3k+1$. The dual graph is the following.
\begin{center}
\includegraphics[scale=0.6]{dual7mod12.pdf}
\end{center}
Black edges have length $6k+3$, cyan edges length $12k+6$, red edges length 2 and green
are of length $1$. As a consequence, we conclude that $l(\Gp)=12k^2+32k+16$. 

\subsection{Case $p=12k+11$}
In this case,  diagram for the special fiber is given by Figure \ref{fig:semistable11}.
Further $g(c_{2,0}) = g(c_{0,2}) = 0, \quad g(c_{1,1}^i) = 3k^2+2k, \quad g(\ell_i) = 6k+5, 
\quad g(e)= 3k+2, \quad g(f) = 2k+1$. The dual graph is the following.
\begin{center}
\includegraphics[scale=0.6]{dual11mod12.pdf}
\end{center}
Black edges have length $6k+5$, orange edges length $18k+15$, cyan edges length $12k+10$, 
blue edges length 3, red edges length 2 and green are of length $1$.
As a consequence, we conclude that $l(\Gp)=12k^2+72k+60$.
